Reach-avoid Verification using Lyapunov Densities

Reach-avoid analysis combines the construction of safety and specific progress guarantees, and is able to formalize many important engineering problems. In this paper we study the reach-avoid verification problem of systems modelled by ordinary differential equations using Lyapunov densities. Firstly, the weak reach-avoid verification is considered. Given an initial set, a safe set and a target set, the weak reach-avoid verification is to verify whether the reach-avoid property (i.e., the system will enter the target set eventually while staying inside the safe set before the first target hitting time) holds for almost all states in the initial set. We propose two novel sufficient conditions using Lyapunov densities for the weak reach-avoid verification. These two sufficient conditions are shown to be weaker than existing ones, providing more possibilities of verifying weak reach-avoid properties successfully. Then, we generalize these conditions to the verification of reach-avoid properties for all states in the initial set. Finally, an example demonstrates theoretical developments of proposed conditions.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> algorithmic.tex <==
% ALGORITHMIC STYLE for LaTeX version 2e
%
% This style file is free software; you can redistribute it and/or
% modify it under the terms of the GNU Lesser General Public
% License as published by the Free Software Foundation; either
% version 2 of the License, or (at your option) any later version.
%
% This style file is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
% Lesser General Public License for more details.
%
% You should have received a copy of the GNU Lesser General Public
% License along with this style file; if not, write to the
% Free Software Foundation, Inc., 59 Temple Place - Suite 330,
% Boston, MA  02111-1307, USA.
%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithmic}[2005/05/08]
\typeout{Document Style `algorithmic' - environment}
%
\RequirePackage{ifthen}
\RequirePackage{calc}
\RequirePackage{keyval}
\newboolean{ALC@noend}
\setboolean{ALC@noend}{false}
\newcounter{ALC@line}
\newcounter{ALC@rem}
\newcounter{ALC@depth}
\newlength{\ALC@tlm}
%
\DeclareOption{noend}{\setboolean{ALC@noend}{true}}
%
\ProcessOptions
%
%
% For indentation of algorithms
\newlength{\algorithmicindent}
\setlength{\algorithmicindent}{0pt}
\def\algsetup{\setkeys{ALG}}
\define@key{ALG}{indent}{\setlength{\algorithmicindent}{#1}}
\ifthenelse{\lengthtest{\algorithmicindent=0pt}}%
{\setlength{\algorithmicindent}{1em}}{}
%
% ALGORITHMIC
\newcommand{\algorithmicrequire}{\textbf{Require:}}
\newcommand{\algorithmicensure}{\textbf{Ensure:}}
\newcommand{\algorithmiccomment}[1]{\{#1\}}
\newcommand{\algorithmicend}{\textbf{end}}
\newcommand{\algorithmicif}{\textbf{if}}
\newcommand{\algorithmicthen}{\textbf{then}}
\newcommand{\algorithmicelse}{\textbf{else}}
\newcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
\newcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
\newcommand{\algorithmicfor}{\textbf{for}}
\newcommand{\algorithmicforall}{\textbf{for all}}
\newcommand{\algorithmicdo}{\textbf{do}}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
\newcommand{\algorithmicwhile}{\textbf{while}}
\newcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
\newcommand{\algorithmicloop}{\textbf{loop}}
\newcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
\newcommand{\algorithmicrepeat}{\textbf{repeat}}
\newcommand{\algorithmicuntil}{\textbf{until}}
\newcommand{\algorithmicprint}{\textbf{print}}
\newcommand{\algorithmicreturn}{\textbf{return}}
\def\ALC@item[#1]{%
\if@noparitem \@donoparitem
  \else \if@inlabel \indent \par \fi
         \ifhmode \unskip\unskip \par \fi
         \if@newlist \if@nobreak \@nbitem \else
                        \addpenalty\@beginparpenalty
                        \addvspace\@topsep \addvspace{-\parskip}\fi
           \else \addpenalty\@itempenalty \addvspace\itemsep
          \fi
    \global\@inlabeltrue
\fi
\everypar{\global\@minipagefalse\global\@newlistfalse
          \if@inlabel\global\@inlabelfalse \hskip -\parindent \box\@labels
             \penalty\z@ \fi
          \everypar{}}\global\@nobreakfalse
\if@noitemarg \@noitemargfalse \if@nmbrlist \refstepcounter{\@listctr}\fi \fi
\sbox\@tempboxa{\makelabel{#1}}%
\global\setbox\@labels
 \hbox{\unhbox\@labels \hskip \itemindent
       \hskip -\labelwidth \hskip -\ALC@tlm
       \ifdim \wd\@tempboxa >\labelwidth
                \box\@tempboxa
          \else \hbox to\labelwidth {\unhbox\@tempboxa}\fi
       \hskip \ALC@tlm}\ignorespaces}
%
\newenvironment{algorithmic}[1][0]{
\setcounter{ALC@depth}{\@listdepth}%
\let\@listdepth\c@ALC@depth%
\let\@item\ALC@item
  \newcommand{\ALC@lno}{%
\ifthenelse{\equal{\arabic{ALC@rem}}{0}}
{{\footnotesize \arabic{ALC@line}:}}{}%
}
\let\@listii\@listi
\let\@listiii\@listi
\let\@listiv\@listi
\let\@listv\@listi
\let\@listvi\@listi
\let\@listvii\@listi
  \newenvironment{ALC@g}{
    \begin{list}{\ALC@lno}{ \itemsep\z@ \itemindent\z@
    \listparindent\z@ \rightmargin\z@ 
    \topsep\z@ \partopsep\z@ \parskip\z@\parsep\z@
    \leftmargin \algorithmicindent%1em
    \addtolength{\ALC@tlm}{\leftmargin}
    }
  }
  {\end{list}}
  \newcommand{\ALC@it}{\addtocounter{ALC@line}{1}\addtocounter{ALC@rem}{1}\ifthenelse{\equal{\arabic{ALC@rem}}{#1}}{\setcounter{ALC@rem}{0}}{}\item}
  \newcommand{\ALC@com}[1]{\ifthenelse{\equal{##1}{default}}%
{}{\ \algorithmiccomment{##1}}}
  \newcommand{\REQUIRE}{\item[\algorithmicrequire]}
  \newcommand{\ENSURE}{\item[\algorithmicensure]}
  \newcommand{\PRINT}{\ALC@it\algorithmicprint{}\ \ }
  \newcommand{\RETURN}{\ALC@it\algorithmicreturn{}\ \ }
  \newcommand{\STATE}{\ALC@it}
  \newcommand{\COMMENT}[1]{\algorithmiccomment{##1}}
  \newenvironment{ALC@if}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@for}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@whl}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@loop}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@rpt}{\begin{ALC@g}}{\end{ALC@g}}
  \renewcommand{\\}{\@centercr}
  \newcommand{\IF}[2][default]{\ALC@it\algorithmicif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSE}[1][default]{\end{ALC@if}\ALC@it\algorithmicelse%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSIF}[2][default]%
{\end{ALC@if}\ALC@it\algorithmicelsif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\FOR}[2][default]{\ALC@it\algorithmicfor\ ##2\ \algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\FORALL}[2][default]{\ALC@it\algorithmicforall\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\WHILE}[2][default]{\ALC@it\algorithmicwhile\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@whl}}
  \newcommand{\LOOP}[1][default]{\ALC@it\algorithmicloop%
\ALC@com{##1}\begin{ALC@loop}}
  \newcommand{\REPEAT}[1][default]{\ALC@it\algorithmicrepeat%
\ALC@com{##1}\begin{ALC@rpt}}
  \newcommand{\UNTIL}[1]{\end{ALC@rpt}\ALC@it\algorithmicuntil\ ##1}
  \ifthenelse{\boolean{ALC@noend}}{
    \newcommand{\ENDIF}{\end{ALC@if}}
    \newcommand{\ENDFOR}{\end{ALC@for}}
    \newcommand{\ENDWHILE}{\end{ALC@whl}}
    \newcommand{\ENDLOOP}{\end{ALC@loop}}
  }{
    \newcommand{\ENDIF}{\end{ALC@if}\ALC@it\algorithmicendif}
    \newcommand{\ENDFOR}{\end{ALC@for}\ALC@it\algorithmicendfor}
    \newcommand{\ENDWHILE}{\end{ALC@whl}\ALC@it\algorithmicendwhile}
    \newcommand{\ENDLOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
  } 
  \renewcommand{\@toodeep}{}
  \begin{list}{\ALC@lno}{\setcounter{ALC@line}{0}\setcounter{ALC@rem}{0}%
    \itemsep\z@ \itemindent\z@ \listparindent\z@%
    \partopsep\z@ \parskip\z@ \parsep\z@%
    \labelsep 0.5em \topsep 0.2em%
\ifthenelse{\equal{#1}{0}}
  {\labelwidth 0.5em }
  {\labelwidth  1.2em }
\leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
    \ALC@tlm\labelsep
  }
}
{\end{list}}


==> controllers.tex <==
\section{Reach-avoid Controllers Synthesis}
It has been widely recognized that density functions are useful to formulate nonlinear control synthesis in terms of convex optimization. In this section we will synthesize weak/strong reach-avoid controllers with the help of constraint \eqref{weak_exponential_con} in Theorem \ref{exponential_almost}.


\subsection{Preliminaries}
In this subsection we introduced controlled continuous-time systems and associated reach-avoid controllers synthesis problems of interest. 

The controlled continuous-time system is a system with a feedback controller  whose dynamics are described by an ODE of the following form:
\begin{equation}
\label{c_sys}
\dot{\bm{x}}(t)=\bm{f}(\bm{x}(t))+\bm{g}(\bm{x}(t)) \bm{u}(\bm{x}(t)),
\bm{x}(0)=\bm{x}_0\in \mathbb{R}^n,
\end{equation}
where $\dot{\bm{x}}(t)=\frac{d \bm{x}(t)}{d t}$, the feedback controller $\bm{u}(\bm{x})\in \mathbb{R}^m$ is locally Lipschitz continuous, and $\bm{f}(\bm{x},\bm{u})=(f_1(\bm{x},\bm{u}),\ldots,f_n(\bm{x},\bm{u}))^{\top}$ with $f_i(\bm{x},\bm{u})\in \mathbb{R}[\bm{x},\bm{u}]$.



%\begin{definition}
%    Given an initial state $\bm{x}_0\in \mathcal{X}$, a reach-avoid feedback controller $\bm{u}(\cdot):\mathbb{R}^n\rightarrow \mathbb{R}^m$ is a controller, which drives the the closed-loop system \eqref{c_sys} to satisfy the reach-avoid property, i.e., system \eqref{c_sys} will enter the target set $\mathcal{X}_r$ in finite time while staying inside the safe set $\mathcal{X}$ before the first target hitting time. 
%\end{definition}


%\begin{definition}[Strong Controlled Reach-avoid Set]
%    Given system \label{c_sys} with the safe set $\mathcal{X}$ and target set $\mathcal{X}_r$, a \textit{strong} controlled reach-avoid set $\mathcal{R}_{s,c}\subseteq \mathcal{X}$ is a set of all initial states such that there exists a feedback controller $\bm{u}(\cdot): \mathcal{R}_{s,c}\rightarrow \mathbb{R}^m$, which drives system \label{c_sys} starting from all of them to enter the target set $\mathcal{X}_r$ in finite time while staying inside $\mathcal{R}_{s,c}$ before the first target hitting time.
%\end{definition}

%\begin{definition}[Weak Controlled Reach-avoid Set]
%Given system \label{c_sys} with the safe set $\mathcal{X}$ and target set $\mathcal{X}_r$, a \textit{weak} controlled reach-avoid set $\mathcal{R}_{w,c}\subseteq \mathcal{X}$ is a set of all initial states such that there exists a feedback controller $\bm{u}(\cdot): \mathcal{R}_{w,c}\rightarrow \mathbb{R}^m$, which drives system \label{c_sys} starting from almost all of them to enter the target set $\mathcal{X}_r$ in finite time while staying inside $\mathcal{R}_{w,c}$ before the first target hitting time.
%\end{definition}



%If the initial set $\mathcal{X}_0$ is a subset of the strong controlled reach-avoid set $\mathcal{R}_{s,c}$ or the weak controlled reach-avoid set $\mathcal{R}_{w,c}$, it is evident that the strong or reach-avoid property holds for system \label{c_sys} with the synthesized feedback reach-avoid controller $\bm{u}(\cdot): \mathcal{R}_{w,c}\rightarrow \mathbb{R}^m$.

A weak/strong feedback reach-avoid controller $\bm{u}(\bm{x})\in \mathbb{R}^m$ is defined in Definition \ref{srac}. 
\begin{definition}[Strong/Weak Reach-avoid Controllers]
\label{srac}
   Given system \label{c_sys} with the safe set $\mathcal{X}$, target set $\mathcal{X}_r$ and initial set $\mathcal{X}_0$, a \textit{weak} (or, \textit{strong}) reach-avoid feedback controller $\bm{u}(\bm{x})\in \mathbb{R}^m$ is a controller, which drives system \label{c_sys} starting from almost all initial states in $\mathcal{X}_0$ (or, all initial states in $\mathcal{X}_0$) to enter the target set $\mathcal{X}_r$ in finite time while staying inside the safe set $\mathcal{X}$ before the first target hitting time.   
\end{definition}

The focus of this section is to synthesize a \textit{weak}(or, \textit{strong}) reach-avoid feedback controller $\bm{u}(\cdot)\in \mathbb{R}^m$.
%\begin{problem}[Reach-avoid Controllers Synthesis Problem]
% Given system \label{c_sys} with the safe set $\mathcal{X}$, target set $\mathcal{X}_r$ and initial set $\mathcal{X}_0$, the reach-avoid  controllers synthesis problem is to synthesize a \textit{weak}(or, \textit{strong}) reach-avoid feedback controller $\bm{u}(\cdot)\in \mathbb{R}^m$.
%\end{problem}

\subsection{Reach-avoid Controllers Synthesis}
\label{uracs}
In this subsection we detail our method of synthesizing strong/weak feedback reach-avoid controllers, chi

Our method is built upon condition \eqref{weak_exponential_con}, which is convex on the pair $(\rho,\rho \bm{u})$. Via introducing $\bm{\psi}=\rho \bm{u}$ as a search variable, we can use convex optimization to find a feasible pair $(\rho,\bm{v})$, and then recover the control law as $\bm{u}(\bm{x})=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})}$. 

\begin{corollary}
 Given $\lambda\in \mathbb{R}$, functions $\rho(\bm{x})\in \mathcal{C}^1(\overline{\mathcal{X}})$ and $\bm{\psi}(\bm{x})\in \mathcal{C}^1(\overline{\mathcal{X}},\mathbb{R}^m)$ satisfying  
\begin{equation}
\label{controllers_syn}
\begin{cases}
&\triangledown\cdot (\rho \bm{f}+ \bm{g}\bm{\psi})(\bm{x})\geq \lambda \rho(\bm{x}), \forall \bm{x}\in \overline{\mathcal{X}\setminus \mathcal{X}_r},\\
& \rho(\bm{x})\leq 0, \forall \bm{x}\in \partial \mathcal{X},\\
&\rho(\bm{x})>0,  \forall \bm{x} \in \mathcal{X}_0,
\end{cases}
\end{equation}
\begin{enumerate}
\item if $\lambda_0<\lambda$, then the feedback controller $\bm{u}(\bm{x}):=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})}$, mapping $\mathcal{R}$ to $\mathbb{R}^m$, is a strong feedback reach-avoid feedback controller;
\item if $\lambda_0>0$ and $0<\lambda\leq \lambda_0$, then the feedback controller $\bm{u}(\bm{x}):=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})}$, mapping $\mathcal{R}$ to $\mathbb{R}^m$, is a weak feedback reach-avoid controller,
\end{enumerate}
where $\mathcal{R}=\{\bm{x}\in \mathcal{X}\mid \rho(\bm{x})>0\}$ and $\lambda_0=\max_{\bm{x}\in \overline{\mathcal{R}\setminus \mathcal{X}_r}}\triangledown (\bm{f}(\bm{x})+\bm{g}(\bm{x}) \bm{u}(\bm{x}))$.
\end{corollary}
\begin{proof}
The conclusion can be obtained via following the proofs of Theorem \ref{exponential_almost} and Corollary \ref{weak_strong_ex}.
\end{proof}

%The difficulty arises because $\bm{u}(\bm{x})$ becomes singular at points where $\rho(\bm{x})=0$, unless $\bm{v}(\bm{x})$ also vanishes there.

%To overcome the difficulty, we will synthesize controllers under the magnitude constraint $|\bm{u}(\bm{x})|\leq c$, where $c>0$, using the conditions
%\begin{equation}
%\label{control_con}
%\begin{cases}
%&\triangledown\cdot [\rho \bm{f}+\bm{v}]\geq \lambda \rho(\bm{x}), \forall \bm{x}\in \overline{\tilde{\mathcal{X}}\setminus \mathcal{X}_r},\\
%& \rho(\bm{x})\leq 0, \forall \tilde{\mathcal{X}}\setminus \mathcal{X}\\
%&\rho(\bm{x})>0,  \forall \bm{x} \in \mathcal{X}_0,\\
%&|\bm{u}(\bm{x})|\leq c \rho(\bm{x}), \forall \bm{x}\in \overline{\tilde{\mathcal{X}}\setminus \mathcal{X}_r}.
%\end{cases}
%\end{equation}
%Given a solution $(\rho, \bm{v})$ to constraint \eqref{control_con}, the control law $\bm{u}(\bm{x})=\frac{\bm{v}(\bm{x})}{\rho(\bm{x})}$ makes $\mathcal{R}=\{\bm{x}\mid \rho(\bm{x})>0\}$ be a weak reach-avoid set.


%Given functions $\alpha(\bm{x})$ and $\beta(\bm{x})$ both of which satisfy 
%$\alpha(\bm{x})\geq 0$ and $\beta(\bm{x})\geq 0$ for $\bm{x} \in \{\bm{x}\in \mathcal{X}\mid \rho(\bm{x})>0\}$, if the functions $\rho(\bm{x})$ and $\bm{v}(\bm{x})$ satisfy the following constraints  
%\begin{equation}
%\label{control_con}
%\begin{cases}
%&\triangledown\cdot [\rho \bm{f}+\bm{v}]\geq \lambda \rho(\bm{x}), \forall \bm{x}\in \overline{\tilde{\mathcal{X}}\setminus \mathcal{X}_r},\\
%& \rho(\bm{x})\leq 0, \forall \tilde{\mathcal{X}}\setminus \mathcal{X}\\
%&\rho(\bm{x})>0,  \forall \bm{x} \in \mathcal{X}_0,\\
%&c \rho(\bm{x})-\bm{u}(\bm{x})\geq \alpha(\bm{x}), \forall \bm{x}\in \overline{\tilde{\mathcal{X}}\setminus \mathcal{X}_r},\\
%&c \rho(\bm{x})+\bm{u}(\bm{x})\geq \beta(\bm{x}), \forall \bm{x}\in \overline{\tilde{\mathcal{X}}\setminus \mathcal{X}_r},
%\end{cases}
%\end{equation}
% the control law $\bm{u}(\bm{x})=\frac{\bm{v}(\bm{x})}{\rho(\bm{x})}$ makes $\mathcal{R}=\{\bm{x}\in \mathcal{X}\mid \rho(\bm{x})>0\}$ be a weak reach-avoid set.

%A special instance of $\alpha(\bm{x})$ is $\lambda_1 \rho(\bm{x})$ with $\lambda_1>0$.   We generally require $\lambda_1<c$. 

Benefiting from constraint \eqref{controllers_syn}, the problem of synthesizing a strong/weak feedback reach-avoid controller can be encoded into a problem of solving a single convex program. 
 If functions $\rho(\bm{x})$ and $\bm{\psi}(\bm{x})$ in \eqref{controllers_syn} are restricted to polynomial functions over $\bm{x}\in \mathbb{R}^n$, we can encode constraint \eqref{controllers_syn} in the form of sum-of-squares constraints and obtain a semi-definite program for synthesizing a strong/weak reach-avoid controller. 


%$\bm{c}\cdot \widehat{\bm{w}}=\int_{\overline{\mathcal{X}}}v(\bm{x})d\bm{x}$, $\widehat{\bm{w}}$ is the constant vector computed by integrating the monomials in $v(\bm{x})\in \mathbb{R}[\bm{x}]$ over $\overline{\mathcal{X}}$, $\bm{c}$ is the vector composed of unknown coffecients in $v(\bm{x})\in \mathbb{R}[\bm{x}]$; 

\begin{remark}
Although constraint \eqref{weak_asympt_con} is also convex on the pair $(\rho_1, \bm{\psi}_1,\rho_2,\bm{\psi}_2)$ with $\bm{\psi}_1=\rho_1\bm{u}$ and $\bm{\psi}_2=\rho_2\bm{u}$, it is challenging to guarantee that 
\[\bm{u}=\frac{\bm{\psi}_1}{\rho_1}=\frac{\bm{\psi}_2}{\rho_2}.\] Therefore, we use constraint \eqref{weak_exponential_con} rather than \eqref{weak_asympt_con} to perform computations in this paper.
\end{remark}


\oomit{\subsection{Constrained Reach-avoid Controllers Synthesis}
\label{cracs}

\begin{corollary}
 Given $\lambda\in \mathbb{R}$, functions $\rho(\bm{x})\in \mathcal{C}^1(\mathbb{R}^n)$ and $\bm{\psi}(\bm{x})=(\psi_1(\bm{x}),\ldots,\psi(\bm{x}))^{\top}\in \mathcal{C}^1(\mathcal{R},\mathbb{R}^m)$ satisfying  
\begin{equation}
\label{controllers_syn}
\begin{cases}
&\triangledown\cdot (\rho \bm{f}+ \bm{g}\bm{\psi})(\bm{x})\geq \lambda \rho(\bm{x}), \forall \bm{x}\in \overline{\mathcal{X}\setminus \mathcal{X}_r},\\
& \rho(\bm{x})\leq 0, \forall \bm{x}\in \partial \mathcal{X},\\
&\rho(\bm{x})>0,  \forall \bm{x} \in \mathcal{X}_0,\\
& \frac{\psi^2_i(\bm{x})}{\rho^2(\bm{x})} \leq U_i, \forall \bm{x}\in \overline{\mathcal{X}},\\
&i=1,\ldots,m,
\end{cases}
\end{equation}
where $\mathcal{R}=\{\bm{x}\in \mathcal{X}\mid \rho(\bm{x})>0\}$,
\begin{enumerate}
\item if $\lambda_0<\lambda$, then the feedback controller $\bm{u}(\bm{x}):=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})}$, mapping $\mathcal{R}$ to $\mathcal{U}$, is a strong feedback reach-avoid feedback controller;
\item if $\lambda_0>0$ and $0<\lambda\leq \lambda_0$, then the feedback controller $\bm{u}(\bm{x}):=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})}$, mapping $\mathcal{R}$ to $\mathcal{U}$, is a weak feedback reach-avoid feedback controller,
\end{enumerate}
where $\lambda_0=\max_{\bm{x}\in \overline{\mathcal{R}\setminus \mathcal{X}_r}}\triangledown (\bm{f}(\bm{x})+\bm{g}(\bm{x}) \bm{u}(\bm{x}))$.
\end{corollary}
\begin{proof}
Constraint $\frac{\psi^2_i(\bm{x})}{\rho^2(\bm{x})} \leq U_i, \forall \bm{x}\in \overline{\mathcal{X}}$($i=1,\ldots,m$) implies that $\bm{u}(\bm{x})=\frac{\bm{\psi}(\bm{x})}{\rho(\bm{x})} \in \mathcal{U}$ over $\overline{\mathcal{X}}$. The conclusion can be obtained via following the proofs of Theorem \ref{exponential_almost} and Corollary \ref{weak_strong_ex}.
\end{proof}

\begin{algorithm}
 %\begin{algorithmic}
\begin{equation}
\label{sos1}
%\begin{split}
%&\max  \bm{c} \cdot \hat{\bm{w}}\\
%&\text{s.t.}\\
\begin{cases}
\triangledown\cdot (\rho \bm{f}+ \bm{g}\bm{\psi})(\bm{x})-\lambda \rho(\bm{x})+s_0(\bm{x}) h(\bm{x})-s_1(\bm{x})g(\bm{x})\in \sum[\bm{x}],\\
\rho(\bm{x})-\epsilon_0+s_3(\bm{x}) l(\bm{x})\in \sum[\bm{x}],\\
-\rho(\bm{x})+p(\bm{x}) h(\bm{x}) \in \sum[\bm{x}],\\
w_i(\bm{x})-s_{4,i}(\bm{x})h(\bm{x}) \in \sum[\bm{x}],\\
U_i-w_i(\bm{x})-s_{5,i}(\bm{x})h(\bm{x}) \in \sum[\bm{x}],\\
\begin{bmatrix}
    w_i(\bm{x})& \psi_i(\bm{x})\\
    \psi_i(\bm{x})&1
\end{bmatrix}
\succcurlyeq 0, \forall \bm{x}\in \overline{\mathcal{X}},\\
\begin{bmatrix}
    w_i(\bm{x})& c_i(\bm{x})\\
    c_i(\bm{x})&\widehat{\rho}(\bm{x}) 
\end{bmatrix}
\succcurlyeq 0, \forall \bm{x}\in \overline{\mathcal{X}}\\
\end{cases}
%\end{split}
\end{equation}
where $\rho(\bm{x}), p(\bm{x}), \bm{\psi}_i(\bm{x})\in \mathbb{R}[\bm{x}]$, and $s_{j}(\bm{x})\in \sum[\bm{x}]$, $i=0,\ldots,3$.
%\end{algorithmic}
\end{algorithm}}


==> relate_work.tex <==
\subsection*{\textbf{Related Work}}
\label{rw}

